Explainable Deep Reinforcement Learning for Portfolio Management: An Empirical Approach

Deep reinforcement learning (DRL) has been widely studied in the portfolio management task. However, it is challenging to understand a DRL-based trading strategy because of the black-box nature of deep neural networks. In this paper, we propose an empirical approach to explain the strategies of DRL agents for the portfolio management task. First, we use a linear model in hindsight as the reference model, which finds the best portfolio weights by assuming knowing actual stock returns in foresight. In particular, we use the coefficients of a linear model in hindsight as the reference feature weights. Secondly, for DRL agents, we use integrated gradients to define the feature weights, which are the coefficients between reward and features under a linear regression model. Thirdly, we study the prediction power in two cases, single-step prediction and multi-step prediction. In particular, we quantify the prediction power by calculating the linear correlations between the feature weights of a DRL agent and the reference feature weights, and similarly for machine learning methods. Finally, we evaluate a portfolio management task on Dow Jones 30 constituent stocks during 01/01/2009 to 09/01/2021. Our approach empirically reveals that a DRL agent exhibits a stronger multi-step prediction power than machine learning methods.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> sections/saved.tex <==
%%====================old paragraph: environment====
%We can use discrete action space to present the input: $\{-k,...,-1, 0, 1, ..., k\}$, it is a $2k+1$ dimensional vector, k must be an integer. $k$ presents the number of shares we buy, $-k$ represents the number of shares we sell, $k\in [1,h_{max}]$, $h_{max}$ is the maximum amount of shares we could buy or sell at each time, it is a predefined parameter. For example, if $k=10$, then the action space is a 21-dimensional vector: $\{-10, -9, -8,...,-1,0,1,...8,9,10\}$. "Buy 10 shares of stock AAPL" or "Sell 10 shares of stock AAPL" are some of the possible actions. We can also use continuous action space to present the input: $\{-k,...,0,..., k\}$, it is a one dimensional vector, k is any real number within $[0,h_{max}]$. 
%The action space for multiple stocks is different from the single stock. In this paper, we use the 30 Dow Jones stocks. For each stock, its continuous action space is: $\{-k,...,-1, 0, 1, ..., k\}$, therefore the action space for 30 stocks is: $30\times\{-k,...,-1, 0, 1, ..., k\}$. There are two factors we need to consider namely Direction and Quantity. Direction is the Buy, Hold, and Sell actions. Quantity is the amount of shares we want to execute subject to the three actions. We use the sign of k 
%\begin{equation}
%sgn(k)=
%\begin{cases}
%  -1, & \text{Sell Action},\  \\
%  0, & \text{Hold Action},\  \\
%  1, & \text{Buy Action}.\  \\
%
%\end{cases}
%\end{equation} to represent the actions. A positive sign of k presents Buy action, a negative sign of k presents Sell action, 0 presents Hold action. The shape of the action space becomes 30, each stock has its own amount of shares $k_{d}$ (where d = 1,...,30) subjects to the Buy and Sell actions, or just hold on current positions. We need to normalize the action space, because for some of the RL algorithms (e.g. A2C or PPO), it defines the policy directly on a Gaussian, the output is not re-scaled to fit the action space limits. If the limits are too big or too small, then the sampled actions will deviate from the limits of the space a lot. So we need to make sure the action space is normalized and symmetric as the initial standard deviation of the Gaussian used to defined the policy \cite{stable-baselines}.

%unnormalized actions space only works with algorithms that don't really directly on a Gaussian to define the policy (e.g. DDPG or SAG, where the output is re-scaled to fit the action space limits). Limits too big, -1000,1000 the sampled actions will only have values around 0 far away from the limits of the space. Limits too small, in that case, the sampled actions will almost always saturate (be greater than the limits)
%best practice: action space is normalized, symmetric and has an interval range of 2, which is usually the same magnitude as the initial standard deviation of the Gaussian used to defined the policy (unit initial std in Stable-Baselines)

%The action space for 30 stock becomes a 30-dimensional vector: $\{k_{1},...,k_{30}\}$. 
%We can also set the maximum and the minimum share we can trade using low and high in space.Box.A positive sign of $k$ indicates an upward direction meaning the stock will go up. A negative sign of $sgn(P_{t+1}-P_{t})$ indicates a downward direction meaning the stock will go down. 0 means the stock price will remain the same. Therefore, a

%The parameters $\theta^\mu$ of the actor network are then as follows:
%\begin{align}
%%    \nabla_{\theta^\mu} J &\approx \mathbb{E}_{s_t,a_t,r_t,s_{t+1}\sim \text{buffer}}
 %   [\nabla_{\theta^\mu} Q(s_t,\mu(s_t|\theta^\mu)|\theta^Q)] \\
 %   & = \mathbb{E}_{s_t,a_t,r_t,s_{t+1}\sim \text{buffer}}
 %   [\nabla_{a} Q(s_t,\mu(s_t)|\theta^Q) \nabla_{\theta^\mu} \mu(s_t|\theta^\mu)].
%\end{align}

%are updated as follows:
%\begin{align}
%    \theta^{Q'} &\leftarrow \tau \theta^Q + (1-\tau)\theta^{Q'},
%    \\
%    \theta^{\mu'} &\leftarrow \tau \theta^\mu + (1-\tau)\theta^{\mu'},
%\end{align} where $\tau$ denotes learning rate. 

%%====================old paragraph: DDPG====
%DDPG is an improved version of Deterministic Policy Gradient (DPG) algorithm \cite{DPG}. DPG combines the frameworks of both Q-learning \cite{Sutton} and policy gradient \cite{PolicyGradient}. Compared with DPG, DDPG uses neural networks as function approximator. The DQN approach, however, is still intractable for this problem due to the large size of the action spaces. Since the feasible trading actions for each stock is in a discrete set, and considering the number of total stocks, the sizes of action spaces grow exponentially, leading to the "curse of dimensionality" \cite{Management}. Hence, the policy gradient based algorithms are proposed to map states to actions to address this issue.

%The Q-learning is essentially a method to learn the environment. Instead of using the expectation of $Q(s_{t+1},a_{t+1})$ to update $Q(s_{t},a_{t})$, Q-learning uses greedy action $a_{t+1}$ that maximizes $Q(s_{t+1},a_{t+1})$ for state $s_{t+1}$, i.e.,
%\begin{equation}
%    \label{Q*}
 %   Q_\pi(s_t,a_t) = \mathbb{E}_{s_{t+1}}[r(s_t,a_t,s_{t+1}) + \gamma  Q_{a_{t+1}\sim \mathop{\argmax}_{a_{t+1}'} Q(s_{t+1},a_{t+1}')} (s_{t+1},a_{t+1})].
%     Q_\pi(s_t,a_t) = \mathbb{E}_{s_{t+1}}[r(s_t,a_t,s_{t+1}) + \gamma  \max_{a_{t+1}}Q (s_{t+1},a_{t+1})].
%\end{equation} 
%We implemented the Q-learning function to create and update a Q-table. To update $Q(s_{t},a_{t})$, we use the Bellman equation:
%\begin{equation}
%    \label{Q*}
%     Q^{new}(s_t,a_t) \leftarrow  Q(s_t,a_t) + \alpha [r(s_t,a_t,s_{t+1}) + \gamma  \max_{a_{t+1}}Q %(s_{t+1},a_{t+1}) - Q(s_t,a_t)].
%\end{equation}

%Q-learning is a value-based Reinforcement Learning algorithm that is used to learn the optimal action-selection policy using a Q-value function. It evaluates which action to take based on an action-value function that determines the value of being in a certain state and taking a certain action at that state. Instead of using the expectation of $Q(s_{t+1},a_{t+1})$ to update $Q(s_{t},a_{t})$, Q-learning uses greedy action $a_{t+1}$ that maximizes $Q(s_{t+1},a_{t+1})$ for state $s_{t+1}$, i.e.,
%\begin{equation}
%    \label{Q*}
%     Q_\pi(s_t,a_t) = \mathbb{E}_{s_{t+1}}[r(s_t,a_t,s_{t+1}) + \gamma  \max_{a_{t+1}}Q (s_{t+1},a_{t+1})].
%\end{equation}
%We implemented the Q-learning function to create and update a Q-table. To update $Q(s_{t},a_{t})$, we use the Bellman equation:
%\begin{equation}
%    \label{Q*}
%     Q^{new}(s_t,a_t) \leftarrow  Q(s_t,a_t) + \alpha [r(s_t,a_t,s_{t+1}) + \gamma  \max_{a_{t+1}}Q %(s_{t+1},a_{t+1}) - Q(s_t,a_t)].
%\end{equation}

%Q-table helps us to find the maximum expected future reward of an action, given a current state. This was a good strategy — however, this is not scalable. The major limitation of Q-learning is that Q-learning only works in environments uses discrete and finite state and action spaces, it might be infeasible to apply the optimal algorithm and learn the full state-action table. 

%With Deep Q-learning Network (DQN), which adopts neural networks to perform function approximation, the states are encoded in value function. Instead of calculating all state-action table, DQN minimizes the mean squared error between the predictions $Q(s_{t},a_{t})$ and targets $r(s_t,a_t,s_{t+1}) + \gamma  \max_{a_{t+1}}Q (s_{t+1},a_{t+1})$, therefore the loss function is:
%\begin{equation}
%    \label{DQN*}
%     L = \mathbb{E}[(r(s_t,a_t,s_{t+1}) + \gamma  \max_{a_{t+1}}Q (s_{t+1},a_{t+1}) - Q(s_t,a_t))^{2}].
%\end{equation}

%$s$, $\mu(s)$, $Q(s, a)$, $a = \mu(s) + \mathcal{N}$
% $\frac{1}{n}\sum_{1}^{n}\nabla \theta_{n}$

%In other words, the huge number of states makes Q-learning very slow to converge.

%In case of discrete problem, there might be the problem that the number of discrete state is huge, e.g., tens of thousand. Even though for discrete problem there exist RL algorithm like Q-learning that converge to the optimal value function, it might be just not feasible to apply such an optimal algorithm due the huge number of state. Here, often continuous RL algorithm can be way to overcome this problem, as the number of parameters of the functions approximators is significantly lower than the number of state.

%experience replay
%\sum_{i=1}^{n} (r^{train}_{t+1} - g_\theta(X^{train}_{t}))^{2}
%disadvantage of DQN
%We back-propagate this loss error back into the neural network, and by using stochastic gradient descent we update the weights according to how much they contributed to the loss error. DQN uses experience replay to overcome the correlated samples problem, because learning from batches of consecutive samples increase variances, hence the learning is inefficient. Experience replay solves this problem by randomly sampling mini-batches of transitions from the saved replay memory.

%Policy gradient session
%DQN can only be used for discrete action spaces, because each output node represents an action, continuous space implies an infinite number of possible actions, we can’t have infinite number of neural networks nodes. Policy gradient uses neural network to model the policy itself. The action a is the random variable and the state s is given. Policy gradient networks output the parameters of any probability distribution which represents the best action a to take under the input state s; 


%%====================old paragraph: A2C====
%A2C algorithm is based on policy gradients. Policy gradient uses neural network to model the policy $\pi_{\theta}$. Policy gradient networks output the parameters of any probability distribution which represents the best action $a$ to take under the input state $s$; The policy gradient method is also the "Actor" part of Actor-Critic methods. The objective function for policy gradient is defined as: 
%\begin{equation}
%    \label{PG_objective}
%     J(\theta) = \mathbb{E}[\sum_{t=1}^{T}r(t+1) | \pi_{\theta}(a_{t}|s_{t})]
%\end{equation} where $r(t+1)$ is the reward received by executing action $a$ given state $s$ at time $t$, $T$ is the terminal time. The objective of a policy is to maximize the cumulative reward received from time $t$ to $T$. By applying the policy gradient theorem \cite{policy_gradient_2000}, which states that the derivative of the expected reward is the expectation of the product of the reward and gradient of the log of the policy $\pi_{\theta}(a_{t}|s_{t})$. we can write the gradient $\nabla J_{\theta}(\theta)$ as:
%\begin{equation}
%    \label{PG_objective}
%     \nabla J_{\theta}(\theta) = \mathbb{E}[\sum_{t=1}^{T} \nabla_{\theta}\log %\pi_{\theta}(a_{t}|s_{t})G_{t}) ]
%\end{equation} 
%Where $G_{t}$ is the sum of future rewards. The sum of future rewards can be replaced with action-value Q.

%\begin{equation}
%    \label{PG_objective}
%     \nabla J_{\theta}(\theta) = \mathbb{E}[\sum_{t=1}^{T}\nabla_{\theta}\log %\pi_{\theta}(a_{t}|s_{t})Q(s_{t},a_{t}) ]
%\end{equation}
%We will weight the log probabilities by advantage instead of future rewards, thus 

%%====================old paragraph: PPO====
%TRPO is introduced to control the policy gradient update and ensure that the new policy will not be too different from the older one. TRPO Objective function is:
%\begin{equation}
%    \label{TRPO}
%     J^{TRPO}(\theta) = \mathbb{E}_{s\sim\rho^{\pi_{\theta{old}}},a\sim\pi_{\theta{old}}}[
%     \frac{\pi_{\theta}(a_{t}|s_{t})}{\pi_{\theta_{old}}(a_{t}|s_{t})}\hat{A}_{\theta_{old}}(s_{t},a_{t})] 
%\end{equation} 
% subject to
%\begin{equation}
%    \label{TRPO_KL}
%    \mathbb{E}_{s\sim\rho^{\pi_{\theta{old}}}}[D_{KL}(\pi_{\theta{old}}(\cdot|S)||\pi_{\theta}(\cdot|S))]\leq %\delta 
%\end{equation} where TRPO maximizes $J^{TRPO}(\theta)$ subject to a trust region constraint which satisfies a special constraint on how close the new and old policies are allowed to be. The constraint is expressed in terms of KL-Divergence to be small enough with a parameter $\delta$. In this way, the old and new policies would not be a huge difference when this hard constraint is met. However, TRPO is relatively sophisticated to implement and not practical for large deep networks.  PPO is introduced to address these problems by using a clipped surrogate objective while retaining similar performance. It  simplifies the algorithm by removing the KL penalty. 
%Therefore, the TRPO objective becomes:
%\begin{equation}
%    \label{TRPO}
%     J^{TRPO}(\theta) = \mathbb{E}[r(\theta)\hat{A}_{\theta_{old}}(s_{t},a_{t})] 
%\end{equation} We need to prevent the extremely large policy updates to control $r(\theta)$. PPO uses a interval $[1-\epsilon,1+\epsilon]$ to force $r(\theta)$ to stay within this bound. $\epsilon$ is an hyperparameter, usually 0.1 or 0.2 that controls the clip range \cite{TRPO_2015}.


%%%%%%%%%%%%%%%%%%Algorithm%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Commented code

\begin{algorithm}[t]
	\caption{A2C algorithm}
	\begin{algorithmic}[1]
	    \STATE Assume global parameters $\theta$ and $\theta_{v}$
	    \STATE Assume thread-specific parameters $\theta'$ and $\theta_{v}'$
	    \STATE Initialize the time step t = 1
		\WHILE{$T\leq T_{MAX}$}
		    \STATE Reset gradients: $d\theta \leftarrow 0$ and  $d\theta_{v} \leftarrow 0$
            \STATE Synchronize thread-specific parameters with global ones: $\theta' = \theta$ and $\theta_{v}' = \theta_{v}$
            \STATE $t_{start} = t$ and sample a starting state $s_{t}$
            \WHILE{$s_{t}!=TERMINAL$ and $t-t_{start}\leq t_{max}$}
                \STATE Perform action $a_{t}$ according to policy $\pi(a_{t}|s_{t}; \theta')$
                \STATE Receive reward $r_{t}$ and new state $s_{t+1}$
                \STATE Update $t \leftarrow t+1$ 
            \ENDWHILE
            \STATE Initialize the variable that holds the return estimation
             \begin{equation}
                R=
                \begin{cases}
                  0, & \text{if $s_{t}$ is TERMINAL}\  \\
                  V(s_{t}, \theta_{v}'), & \text{otherwise}
                \end{cases}
              \end{equation}
             \FOR{$i = t-1,...,t_{start}$}
                \STATE $R \leftarrow \gamma R + r_{i}$
                \STATE Accumulate gradients w.r.t. $\theta':$
                \begin{equation}
                    d\theta \leftarrow d\theta+\nabla_{\theta'}\log\pi(a_{i}|s_{i};\theta')(R-V(s_{t};\theta_{v}'))
                \end{equation}
                \STATE Accumulate gradients w.r.t. $\theta_{v}':$
                \begin{equation}
                    d\theta_{v} \leftarrow d\theta_{v}+\partial(R-V(s_{t};\theta_{v}'))^2/\partial\theta_{v}'
                \end{equation}
             \ENDFOR
             \STATE Update synchronously $\theta$ using $d\theta$ and $\theta_{v}$ using $d\theta_{v}$.
             \STATE Update $T \leftarrow T+1$
        \ENDWHILE
	\end{algorithmic}
	\vspace{-2pt}
	\label{a2c}
\end{algorithm}


\begin{algorithm}[t]
	\caption{DDPG algorithm}
	\begin{algorithmic}[1]
		\STATE Randomly initialize critic network $Q(s,a|\theta^Q)$ and actor $\mu(s|\theta^\mu)$ with random weight $\theta^Q$ and $\theta^\mu$;
        \STATE Initialize target network $Q'$ and $\mu' $ with weights $\theta^{Q'} \leftarrow \theta^{Q}$, $\theta^{\mu'} \leftarrow \theta^{\mu}$;
        \STATE Initialize replay buffer $R$;
        \FOR {episode= 1, $M$}
            \STATE Initialize a random process $\mathcal{N}$ for action exploration;
            \STATE Receive initial observation state $s_1$;
            \FOR{t = 1, $T$}
                \STATE {Select action $a_t = \mu(s_t|\theta^\mu) + \mathcal{N}_t$ according to the current policy and exploration noise;}
                \STATE {Execute action $a_t$ and observe reward $r_t$ and state $s_{t+1}$};
                \STATE {Store transition ($s_t$, $a_t$, $r_t$, $s_{t+1})$ in $R$;}
                \STATE {Sample a random minibatch of $N$ transitions ($s_i$ , $a_i$ , $r_i$ , $s_{i +1}$) from $R$;}
                \STATE {Set $y_i = r_i+\gamma Q' (s_{t+1}, \mu' (s_{i+1}|\theta^{\mu'}|\theta^{Q'}))$;}
                \STATE {Update critic by minimizing the loss: $L = \frac{1}{N}\sum_i(y_i -Q(s_i,a_i|\theta^Q))^2$;}
                \STATE {Update the actor policy by using the sampled policy gradient:
                $$
                    \nabla_{\theta^\mu} J\approx \frac{1}{N}\sum_i \nabla_a Q(s,a|\theta^Q)|_{s = s_i,a = \mu(s_i)} \nabla_{\theta^\mu} \mu(s|\theta^\mu)|_{s_i};
                $$}
                \STATE Update the target networks:
                $$\theta^{Q'} \leftarrow \tau \theta^Q + (1-\tau)\theta^{Q'},
                $$ $$
                \theta^{\mu'} \leftarrow \tau \theta^\mu + (1-\tau)\theta^{\mu'}.
                $$
            \ENDFOR
        \ENDFOR
	\end{algorithmic}
	\vspace{-2pt}
	\label{ddpg}
\end{algorithm}


\begin{algorithm}[t]
	\caption{PPO with Clipped Objective}
	\begin{algorithmic}[1]
		\STATE Input: initialize policy parameters $\theta_{0}$, initial value function parameters $\phi_{0}$, clipping threshold $\epsilon$
        \FOR {$k= 1,2,...$}
            \STATE Collect set of partial trajectories $\mathcal{D}_{k} = {\tau_{i}}$ by running policy $\pi_{k} = \pi(\theta_{k})$ in the environment.
            \STATE Compute rewards-to-go $\hat{R}_{t}$
            \STATE Compute advantage estimates $\hat{A}_{t}$ using any advantage estimation algorithm based on the current value function $V_{\phi_{k}}$
            \STATE Compute policy update by maximizing the PPO with clipped objective:
             $$
                \theta_{k+1} = arg\underset{\theta}{max}\mathcal{L}^{CLIP}_{\theta_{k}}(\theta)
             $$
             by taking K steps of minibatch SGD (via Adam), where
             $$
                \mathcal{L}^{CLIP}_{\theta_{k}}(\theta) = \underset{\tau\sim\pi_{k}}{\mathbb{E}}\left[\sum_{t=0}^{T}[min(r_{t}(\theta)\hat{A}_{t}^{\pi_{k}}, clip(r_{t}(\theta), 1-\epsilon,1+\epsilon)\hat{A}_{t}^{\pi_{k}})]\right]
            $$
        \ENDFOR
	\end{algorithmic}
	\vspace{-2pt}
	\label{ppo}
\end{algorithm}
\end{comment}
%%%%%%%%%%%%%%%%%%Algorithm%%%%%%%%%%%%%%%%%%%%%%%%%%
